Recovery Bounds on Class-Based Optimal Transport: A Sum-of-Norms Regularization Framework

We develop a novel theoretical framework for understating OT schemes respecting a class structure. For this purpose, we propose a convex OT program with a sum-of-norms regularization term, which provably recovers the underlying class structure under geometric assumptions. Furthermore, we derive an accelerated proximal algorithm with a closed-form projection and proximal operator scheme, thereby affording a more scalable algorithm for computing optimal transport plans. We provide a novel argument for the uniqueness of the optimum even in the absence of strong convexity. Our experiments show that the new regularizer not only results in a better preservation of the class structure in the data but also yields additional robustness to the data geometry, compared to previous regularizers.

==> Intro_old.tex <==
Optimal Transport (OT), first proposed by Monge as an analysis problem  \cite{monge1781memoire}, has become a classic topic in probability and statistics for transferring mass from one probability distribution to another \cite{villani2008optimal,santambrogio2015optimal}. The OT problem seeks to find a transport map from a source distribution to a target distribution while minimizing the cost of the transport. 
%(see section~\ref{sec:optT} for a precise statement). 
As a richly adopted framework in many different disciplines, OT has also recently been very successfully used in many applications in computer vision, texture analysis, tomographic reconstruction and clustering, as documented in the recent surveys \cite{KPTSR17} and \cite{Sol18}. In many of these applications, OT exploits the geometry of the underlying spaces to effectively yield improved performance over the alternative of obviating it. This improvement, however, comes at a significant computational cost when solving the OT problem. Much attention has  focused on efficient computational and numerical algorithms for OT, and a monograph focusing on this topic appeared \cite{CP18}. In \cite{pmlr-v108-guo20a}, an "accelerated primal-dual randomized coordinate descent (APDRCD)" algorithm is developed to solve the OT problem. An upper bound is also provided for the complexity of the algorithm and it is shown that it could be used for large-scale purposes. 

Several advances in computational approaches to OT have been made in  recent years, primarily focusing on applications in domain adaptation. In \cite{CFTR17}, a generalized conditional gradient method is used to compute OT with the help of a couple of regularizers. Cuturi introduced an entropic regularizer and showed that its adoption with the Sinkhorn algorithm yields a fast computation of OT \cite{cuturi2013sinkhorn}; a theoretical guarantee that the Sinkhorn iteration computes the approximation in near linear time was also provided by \cite{AWR17}. Screenkhorn algorithm proposed in \cite{screenkhorn2019} performs screening to eliminate (and accelerate) the solution of the Sinkhorn algorithm. Another computational breakthrough was achieved by \cite{GCPB16} who gave a stochastic incremental algorithm to solve the entropic regularized OT problem. 
%However, their algorithm works on the dual and semi--dual formulations and while it computes the optimal value, it is not clear how to recover the corresponding optimal coupling. The explicit coupling is needed in order to compute the transport map necessary for many applications such as domain adaptation as in \cite{perrot2016mapping}. 

While the entropic regularization of OT has attracted a lot of attention on account of its many merits, it has some limitations, such as the blurring in the optimal transportation plan induced by the entropy term. An intrinsic property of the entropy term is that it keeps the transportation plan strictly positive and therefore completely dense, unlike unregularized OT. This lack of sparsity can be problematic for applications such as domain adaptation \cite{CFTR17} where the optimal transportation plan is itself of interest and a class structure is present in the data. In this case, an ideal transport plan maps each  class in the source domain to its corresponding class in the target domain. In practice, we should transfer one source class to as few target classes as possible. An amelioration of this effect may be achieved by using a small regularization so long as it is carefully engineered, which is generally difficult.

A case for exploring new regularizers was made in \cite{CFTR17} in the context of domain adaptation applications. In \cite{blondel18a} the primal and dual formulations of OT are regularized with a strongly convex term, and the constraints are relaxed with smooth approximations. \cite{Dessein18} also propose a framework to solve discrete optimal transport problems with smooth convex regularization. The L2 regularization of OT plan also yields a sparse plan. It has notably been used in a doubly stochastic scheme in \cite{seguy2018large}. While promoting sparsity in the transport plan, these techniques are not tailored to the underlying class structure of the data, which may not be known in advance. In this paper, we accordingly propose a novel approach of class--based regularization of the OT problem, based on the recently proposed convex clustering framework of Sum of Norms (SON) \cite{LOL11,HVBJ11}, which presents an improvement on the state of the art on at least two grounds:

{\bf SON Regularizer Benefits for OT}: The SON regularization allows one to discover and exploit the class structure and to preserve the sparsity of the transport plan. While this approach may be superficially reminiscent of a Laplacian regularizer \cite{CFTR17}, the latter only acts indirectly on the transported points  and is quadratic in nature, in contrast to our transport plan. This difference is clearly illustrated in the experiments.
We theoretically show and experimentally validate that this formulation ensures a  transport plan adhering to the class structure. In the source domain, the class structure is given by the labels while it is latent (hidden) in the target domain.  We further show that our formulation leads to the discovery of the underlying hidden class structure in the target domain, and provide for the first time, rigorous guarantees on the recovery of class structure.  No such results, to the best of our knowledge, are known for other regularizers. We also experimentally show that our regularizer does not only yield a better class structure preservation, but also provides additional robustness compared to other class-based regularizers in \cite{CFTR17}.

{\bf Computational Benefits of Stochastic Proximal Algorithm}: Our SON regularizer-based formulation also enjoys computational benefits -- we propose a scalable stochastic incremental algorithm which operates in the primal formulation and explicitly produces the optimal coupling. In contrast to \cite{CFTR17} where full gradients are used, our algorithm operates  in a stochastic incremental framework. Proximal method has been used in OT but not in a stochastic scheme. Examples include \cite{pmlr-alvarez-melis18a} that uses notions of sub-modularity and also \cite{otproximalsplitting}. We first construct an abstract stochastic framework that is based on a combination of proximal and projection iterations
%-- since projection is a special case of proximal operators, this is a very natural combination. However, projection operators lack properties generally assumed for the convergence of stochastic proximal schemes and the combination of the two operators has not been sufficiently discussed in the existing literature. We propose a novel scheme for combining proximal and projection operators
, for which we give a generic proof of convergence at rate $O(1/T)$. We also demonstrate its stability in a number of experiments. We subsequently specialize this general scheme 
for our SON regularizer-based formulation,
%by computing the proximal operator corresponding to our OT formulation in closed form. We derive sparse variants of our algorithms which exploit the fact that each term in the optimization only depends on very few coordinates. Together with using efficient projections to the simplex, 
which leads to an algorithm with  computationally low-cost iterations. Beyond the proposed SON-based framework, our proximal scheme can be used to avoid the reported convergence difficulties gradient-based methods \cite{PN18}.
 %We also use the optimal coupling to compute a transport map which can be used to map out--of--sample points as suggested in \cite{perrot2016mapping}. 
%We improve on \cite{perrot2016mapping} in two ways: (1) while \cite{perrot2016mapping} is limited to linear and kernelized maps, we compute a general non--linear transport map and (2) our transport map works with a general (differentiable) cost function, not only the Euclidean distance as in \cite{perrot2016mapping}.
%\iffalse


It is notable that our formulation differs from the \emph{partial domain adaption} \cite{Cao-pda} and \emph{robust domain adaption} \cite{Balaji2020RobustOT} settings developed to deal with outlier classes or samples. The former assumes some special form of relationship between the source and target classes, whereas, we do not make such assumptions. Furthermore, the partial domain adaptation literature has not been developed yet around the idea of optimal transport. However, we observe that our framework is able to address the partial domain adaptation task, though it is not specialized for this purpose.
The latter proposes a new formulation for OT to reduce the sensitivity to outlier samples. It does not take the class structure in source and target into account. 

{\bf Summary of contributions}: Our main contributions can be summarized as follows:
% \begin{itemize}
% \item We propose in Section~\ref{sec:regson} a new regularized formulation of OT that promotes the sparsity of the transport plan, thereby ensuring a preservation of a class structure typically arising in domain adaptation problems.
% \item In Section~\ref{sec:uniqueness}, we develop a new proof for the uniqueness of the solution optimum of our convex formulation in spite  of its non-strong convexity. We believe that this proposed technique may have wider applicability.
% \item We develop in Section~\ref{sec:alg} a general accelerated stochastic incremental proximal-projection optimization scheme, for which 
% %We derive a novel acceleration scheme for variance reduction in the stochastic projection steps. 
% we give a proof of convergence at a rate $O(1/T)$ without a decaying step size. We specialize the general scheme with an explicit closed form of proximal operators and fast projections to yield a scalable stochastic incremental algorithm for computing our OT formulation, thus producing an optimal coupling (transport plan) explicitly.
% \item We derive the first rigorous results for recovering an OT plan that respects class structure, introduced in Section~\ref{sec:theory} with details in the appendix \ref{theory:class_based}.
% \item Finally in Section~\ref{sec:exp}, we investigate the algorithm on several synthetic and benchmark data sets, and demonstrate the benefits of the new regularizer.
% %\item We construct a general non--linear transport map for an arbitrary differentiable cost function approximating the Barycentric mapping associated with an optimal transport plan. This improves the recent results of \cite{perrot2016mapping} who consider limited classes of mappings and only Euclidean distance.

% \end{itemize}
%\fi
\noindent
i.We propose in Section~\ref{sec:regson} a new regularized formulation of OT that promotes the sparsity of the transport plan, thereby ensuring a preservation of a class structure typically arising in domain adaptation problems.\\
ii. In Section~\ref{sec:uniqueness}, we develop a new proof for the uniqueness of the solution optimum of our convex formulation in spite  of its non-strong convexity. We believe that this proposed technique may have wider applicability.\\
iii. We develop in Section~\ref{sec:alg} a general accelerated stochastic incremental proximal-projection optimization scheme, for which 
%We derive a novel acceleration scheme for variance reduction in the stochastic projection steps. 
we give a proof of convergence at a rate $O(1/T)$ without a decaying step size. We specialize the general scheme with an explicit closed form of proximal operators and fast projections to yield a scalable stochastic incremental algorithm for computing our OT formulation, thus producing an optimal coupling (transport plan) explicitly.\\
iv. We derive the first rigorous results for recovering an OT plan that respects class structure, introduced in Section~\ref{sec:theory} with details in the appendix \ref{theory:class_based}.\\
v. Finally in Section~\ref{sec:exp}, we investigate the algorithm on several synthetic and benchmark data sets, and demonstrate the benefits of the new regularizer.
%\item We construct a general non--linear transport map for an arbitrary differentiable cost function approximating the Barycentric mapping associated with an optimal transport plan. This improves the recent results of \cite{perrot2016mapping} who consider limited classes of mappings and only Euclidean distance.



==> intro_new.tex <==
Machine learning (ML) is based on a close statistical relation between the training samples and the domain of application, or the testing samples. In real world, however, there is a natural discrepancy between the two; a phenomenon  widely referred to as the \emph{domain shift} problem. 
%In the recent years, there has been a rising interest in mitigating the domain shift. 
Domain adaptation is a popular data-driven framework to mitigate the domain shift problem%, which has received an increasing attention, in the recent years. In domain adaptation
, where two separate sets of training samples are assumed: the target domain $\calT$, drawn from a probability measure $\mu$ which is  similar to the testing samples, and the source domain $\calS$ drawn from another distribution $\nu$ with a potential domain shift. For simplicity, we assume that both domains, hence $\mu,\nu$ are defined on $\bbR^d$ for a dimension $d$.

In a realistic scenario, the number $m=|\calS|$ of samples in $\calS$ is comparable or larger than the number $n=|\calT|$ of samples in $\calT$. In domain adaptation, a so-called transport map $T:\calX\to\calX$ is obtained from the data, adapting the source samples to the target domain, and the transported samples $\calS'=T(\calS)$ can be  conveniently mixed with the target samples  to substantially improve the ML task. In mathematical terms, the push-forward measure $\nu'=T\sharp\nu$ of $\nu$ is intended to be as similar to $\mu$ as possible.

The main goal of this paper is to theoretically investigate domain adaptation when a common hidden class structures is present in both domains $\calS,\calT$. Specifically,  we consider a scenario where the source and target domains are both well-partitioned and there exists an inherent correspondence between the partitions in the two domains. Examples of such a setup are abundant [COMPLETE THIS SENTENCE]. In these applications the class structure can be exploited to improve the machine learning task. Accordingly, we develop a theoretical framework for class-based domain adaptation, which includes algorithms respecting the common class structure, without a-priori knowledge of the clusters. In other words, we investigate methods that provably ensure  each source sample being transported to its corresponding partition in the target domain. In this way, we obtain for the first time theoretical results on the benefits of hidden class structure in the domain adaptation problem. 

Our main focus in this paper is on a novel two-stage scheme for the above class-based domain adaptation problem, where in the first stage, clusters in the two domain and their correspondence are discovered. The second stage applies an off-the-shelf domain adaptation technique to each individual cluster. For the first stage, we introduce a novel convex optimization framework combining two well known techniques, namely optimal transport (OT) for domain adaptation and sum-of-norms (SON) clustering. First proposed by Monge as an analysis problem  \cite{monge1781memoire}, OT has become a classic topic in probability and statistics for transferring mass from one probability distribution to another \cite{villani2008optimal,santambrogio2015optimal}. 
A linear programming relaxation of the OT problem, known as the Kantorovich relaxation has gain popularity for domain adaptation. 
%(see section~\ref{sec:optT} for a precise statement). 


{\bf SON Regularizer Benefits for OT}: The SON regularization allows one to discover and exploit the class structure and to preserve the sparsity of the transport plan. While this approach may be superficially reminiscent of a Laplacian regularizer \cite{CFTR17}, the latter only acts indirectly on the transported points  and is quadratic in nature, in contrast to our transport plan. This difference is clearly illustrated in the experiments.
We theoretically show and experimentally validate that this formulation ensures a  transport plan adhering to the class structure. In the source domain, the class structure is given by the labels while it is latent (hidden) in the target domain.  We further show that our formulation leads to the discovery of the underlying hidden class structure in the target domain, and provide for the first time, rigorous guarantees on the recovery of class structure.  No such results, to the best of our knowledge, are known for other regularizers. We also experimentally show that our regularizer does not only yield a better class structure preservation, but also provides additional robustness compared to other class-based regularizers in \cite{CFTR17}.

{\bf Computational Benefits of Stochastic Proximal Algorithm}: Our SON regularizer-based formulation also enjoys computational benefits -- we propose a scalable stochastic incremental algorithm which operates in the primal formulation and explicitly produces the optimal coupling. In contrast to \cite{CFTR17} where full gradients are used, our algorithm operates  in a stochastic incremental framework. Proximal method has been used in OT but not in a stochastic scheme. Examples include \cite{pmlr-alvarez-melis18a} that uses notions of sub-modularity and also \cite{otproximalsplitting}. We first construct an abstract stochastic framework that is based on a combination of proximal and projection iterations
%-- since projection is a special case of proximal operators, this is a very natural combination. However, projection operators lack properties generally assumed for the convergence of stochastic proximal schemes and the combination of the two operators has not been sufficiently discussed in the existing literature. We propose a novel scheme for combining proximal and projection operators
, for which we give a generic proof of convergence at rate $O(1/T)$. We also demonstrate its stability in a number of experiments. We subsequently specialize this general scheme 
for our SON regularizer-based formulation,
%by computing the proximal operator corresponding to our OT formulation in closed form. We derive sparse variants of our algorithms which exploit the fact that each term in the optimization only depends on very few coordinates. Together with using efficient projections to the simplex, 
which leads to an algorithm with  computationally low-cost iterations. Beyond the proposed SON-based framework, our proximal scheme can be used to avoid the reported convergence difficulties gradient-based methods \cite{PN18}.
 %We also use the optimal coupling to compute a transport map which can be used to map out--of--sample points as suggested in \cite{perrot2016mapping}. 
%We improve on \cite{perrot2016mapping} in two ways: (1) while \cite{perrot2016mapping} is limited to linear and kernelized maps, we compute a general non--linear transport map and (2) our transport map works with a general (differentiable) cost function, not only the Euclidean distance as in \cite{perrot2016mapping}.
%\iffalse


It is notable that our formulation differs from the \emph{partial domain adaption} \cite{Cao-pda} and \emph{robust domain adaption} \cite{Balaji2020RobustOT} settings developed to deal with outlier classes or samples. The former assumes some special form of relationship between the source and target classes, whereas, we do not make such assumptions. Furthermore, the partial domain adaptation literature has not been developed yet around the idea of optimal transport. However, we observe that our framework is able to address the partial domain adaptation task, though it is not specialized for this purpose.
The latter proposes a new formulation for OT to reduce the sensitivity to outlier samples. It does not take the class structure in source and target into account. 

{\bf Summary of contributions}: Our main contributions can be summarized as follows:
% \begin{itemize}
% \item We propose in Section~\ref{sec:regson} a new regularized formulation of OT that promotes the sparsity of the transport plan, thereby ensuring a preservation of a class structure typically arising in domain adaptation problems.
% \item In Section~\ref{sec:uniqueness}, we develop a new proof for the uniqueness of the solution optimum of our convex formulation in spite  of its non-strong convexity. We believe that this proposed technique may have wider applicability.
% \item We develop in Section~\ref{sec:alg} a general accelerated stochastic incremental proximal-projection optimization scheme, for which 
% %We derive a novel acceleration scheme for variance reduction in the stochastic projection steps. 
% we give a proof of convergence at a rate $O(1/T)$ without a decaying step size. We specialize the general scheme with an explicit closed form of proximal operators and fast projections to yield a scalable stochastic incremental algorithm for computing our OT formulation, thus producing an optimal coupling (transport plan) explicitly.
% \item We derive the first rigorous results for recovering an OT plan that respects class structure, introduced in Section~\ref{sec:theory} with details in the appendix \ref{theory:class_based}.
% \item Finally in Section~\ref{sec:exp}, we investigate the algorithm on several synthetic and benchmark data sets, and demonstrate the benefits of the new regularizer.
% %\item We construct a general non--linear transport map for an arbitrary differentiable cost function approximating the Barycentric mapping associated with an optimal transport plan. This improves the recent results of \cite{perrot2016mapping} who consider limited classes of mappings and only Euclidean distance.

% \end{itemize}
%\fi
\noindent
i.We propose in Section~\ref{sec:regson} a new regularized formulation of OT that promotes the sparsity of the transport plan, thereby ensuring a preservation of a class structure typically arising in domain adaptation problems.\\
ii. In Section~\ref{sec:uniqueness}, we develop a new proof for the uniqueness of the solution optimum of our convex formulation in spite  of its non-strong convexity. We believe that this proposed technique may have wider applicability.\\
iii. We develop in Section~\ref{sec:alg} a general accelerated stochastic incremental proximal-projection optimization scheme, for which 
%We derive a novel acceleration scheme for variance reduction in the stochastic projection steps. 
we give a proof of convergence at a rate $O(1/T)$ without a decaying step size. We specialize the general scheme with an explicit closed form of proximal operators and fast projections to yield a scalable stochastic incremental algorithm for computing our OT formulation, thus producing an optimal coupling (transport plan) explicitly.\\
iv. We derive the first rigorous results for recovering an OT plan that respects class structure, introduced in Section~\ref{sec:theory} with details in the appendix \ref{theory:class_based}.\\
v. Finally in Section~\ref{sec:exp}, we investigate the algorithm on several synthetic and benchmark data sets, and demonstrate the benefits of the new regularizer.
%\item We construct a general non--linear transport map for an arbitrary differentiable cost function approximating the Barycentric mapping associated with an optimal transport plan. This improves the recent results of \cite{perrot2016mapping} who consider limited classes of mappings and only Euclidean distance.



==> theory.tex <==
In the appendix (section \ref{theory:class_based}), we show that our SON regularizer is able to \emph{provably} compute transport plans that respect the class structure in the manner, explained in section \ref{sec:regson}. Our approach is to analyse it under a setting such as the well known \emph{stochastic block model} (SBM) \cite{HLL83,SN97}, also known as the \emph{planted partition model} \cite{CK01} which has been used widely as a canonical generative model for the data with clear class structure. In this model, we already have a latent ground truth for the class structure which the algorithm is supposed to recover.

In the supervised version of the domain adaptation problem, the class structure is  given explicitly in the source via the labels, but not in the target domain. In the unsupervised version, the class structure is unknown in both domains. In both cases, it is reasonable to assume that a latent (hidden) class structure exists. We show that our algorithm can discover this hidden class structure in both domains (unsupervised) or in the target (supervised) and computes a transport plan that respects the class structure in the two domains. 





% \section{Proof of Theorem \ref{lemma:resistance}}
% \begin{proof}
% Suppose that there exists a different optimal point $\bX^\prime$. Take $\bD_0=\frac{\bX_0-\bX^\prime}{\|\bX_0-\bX^\prime\|}$, $r=\|\bX_0-\bX^\prime\|$ and $\tlbD=\epsilon\bD_0$ for arbitrary $\epsilon>0$. Further, define $\calN$ as the ball of radius $\delta=r/2$ centered at $\bX_0$. Note that for each $\bY\in \calN$ we have 
% \[
% \scrF(\bY)+\langle\tlbD,\bY\rangle\geq
% \scrF(\bX_0)+\langle\tlbD,\bY\rangle
% =\scrF(\bX^\prime)+\langle\tlbD,\bX^\prime\rangle+\langle\tlbD,(\bY-\bX_0)+(\bX_0-\bX^\prime)\rangle.
% \]
% Now, note that
% $
% \langle\tlbD,(\bY-\bX_0)+(\bX_0-\bX^\prime)\rangle\geq -\delta\epsilon+r\epsilon>0,
% $
% which establishes
% \[
% \scrF(\bY)+\langle\tlbD,\bY\rangle>
% \scrF(\bX^\prime)+\langle\tlbD,\bX^\prime\rangle.
% \]
% Hence,
% $
% \calN\cap\arg\minl_{\bX\in\scrS}\scrF(\bX)+\langle\tlbD,\bX\rangle=\emptyset
% $ and
% since $\epsilon=\|\tlbD\|$ is arbitrarily small, we conclude that $\bX_0$ is not a resistant optimal point. This contradicts the assumption and shows that the solution is unique.  
% \end{proof} 

% \section{Proof of Theorem \ref{thm3:resistant}}
% \begin{proof}
% Denote the optimal point by $\bX^*$. By strong convexity, there exists a $\gamma>0$ such that for any feasible point $\bX\in\scrS$, we have $\scrF(\bX)-\scrF(\bX^*)\geq\frac\gamma 2\|\bX-\bX^*\|_\mathrm{F}^2$. Take $\scrG=\scrF+\langle\tlbD,\bX\rangle$ and note that $\scrG(\bX)-\scrG(\bX^*)\geq\frac\gamma 2\|\bX-\bX^*\|_\mathrm{F}^2+\langle\tlbD,\bX-\bX^*\rangle\geq \frac\gamma 4\|\bX-\bX^*\|_\mathrm{F}^2-\frac 2{\gamma}\|\tlbD\|_\mathrm{F}^2$. This shows that $\scrG>\scrG(\bX^*)$ and hence does not have any global optimal point outside the closed sphere $\{\bX\mid\|\bX-\bX^*\|_\mathrm{F}\leq\frac{\sqrt 8}\gamma\|\tlbD\|_\mathrm{F}\}$. Since $\scrG$ is continuous, it also attains a minimum inside the sphere, which then becomes the global optimal point. We conclude that for any $\epsilon>0$, taking $\|\tlbD\|<\frac{\gamma\epsilon}{\sqrt{8}}$ leads to an optimal solution inside a ball of radius $\epsilon$ centered at $\bX^*$. This shows that the solution is resistant. 
% \end{proof}

% \section{Proof of Theorem \ref{lem:proxop}}
% \begin{proof}
% % * <panahi1986@gmail.com> 2017-11-08T17:23:55.167Z: I can make this proof more detailed
% %
% % ^.
% The proximal operator of $\phi_{k,\bzeta,\bmeta}$ is defined as
% \begin{equation}\label{eq:sthh}
% %\Pi_{\mu,\rho,\bzeta,\bmeta}(\bp,\bq)=
% \underset{(\bx,\by)\in\bbR^m\times\bbR^m}{\mathrm{argmin}}\frac 1{2\mu}\|\bx-\bp\|_2^2+
% \frac 1{2\mu}\|\by-\bq\|_2^2+\phi_{\rho,\bzeta,\bmeta}(\bx,\by).
% \end{equation}
% We introduce a change of variables by $\bu=\nicefrac{(\bx+\by)}{2},
% \bv=\nicefrac{(\bx-\by)}{2}$. First note that $\|a\|^2+\|b\|^2=(\|a+b\|^2+\|a-b\|^2)/2$. Hence
% \[
% \frac 1{2\mu}\|\bx-\bp\|_2^2+
% \frac 1{2\mu}\|\by-\bq\|_2^2=
% \]
% \[
% \frac 1{\mu}\left(\left\|\bu-\frac{\bp+\bq}2\right\|^2+\left\|\bv-\frac{\bp-\bq}2\right\|^2\right)
% \]
% Furthermore,
% \[
% \langle\bx,\bzeta\rangle+\langle\by,\bmeta\rangle=\langle\bu+\bv,\bzeta\rangle+\langle\bu-\bv,\bmeta\rangle=\langle\bu,\bzeta+\bmeta\rangle+\langle\bv,\bzeta-\bmeta\rangle
% \]
% Hence \eqref{eq:sthh} can be written as
% \begin{equation}
% \begin{aligned}
% \label{eq:sth}
% %\Pi_{\mu,\rho,\bzeta,\bmeta}(\bp,\bq)=
% &\underset{(\bu,\bv)\in\bbR^m\times\bbR^m}{\mathrm{argmin}}\frac 1{\mu}\left(\left\|\bu-\frac{\bp+\bq}2\right\|^2+\left\|\bv-\frac{\bp-\bq}2\right\|^2\right)+\\\\
% &\langle\bu,\bzeta+\bmeta\rangle+\langle\bv,\bzeta-\bmeta\rangle+2\rho\|\bv\|_2
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% %\Pi_{\mu,\rho,\bzeta,\bmeta}(\bp,\bq)=
% &=\underset{(\bu,\bv)\in\bbR^m\times\bbR^m}{\mathrm{argmin}}\frac 1{\mu}\left(\left\|\bu-\frac{\bp+\bq-\mu\bzeta-\mu\bmeta}2\right\|^2\right) + \\
% &\frac 1{\mu}\left(
%  \left\|\bv-\frac{\bp-\bq-\mu\bzeta+\mu\bmeta}2\right\|^2\right)+2\rho\|\bv\|_2
% \end{aligned}
% \end{equation}

% This is separable  over
% $\bu$ and $\bv$, and can be analytically solved. We get 
% \[
% \bu=\frac{\bp+\bq-\mu\bzeta-\mu\bmeta}2,\quad \bv=\calT_{\mu\rho}\left(\frac{\bp-\bq-\mu\bzeta+\mu\bmeta}2\right)
% \]
% The result is obtained by setting $\bx=\bu+\bv,\by=\bu-\bv$.
% \end{proof}
% \section{Just-in-Time (JiT) Update}
% \label{sec:jit}
% Here we explain more details about the JiT procedure, explained in section \ref{sec:proxop}. In our problem, each term $\phi_n(x)$ and constraint $S_m$ only involves a small subset $x_{I_n}:= (x_i, i \in I_n)$ of the variables, where $I_n \subseteq [D]$. Hence, the projection and proximal operators alter only a small subset of variables, dramatically reducing the amount of computation. We exploit this to give an algorithm that has much cheaper per-iteration cost. Note that the vanilla algorithm explained in \eqref{eq:alg1} and \eqref{eq:alg2} still operates on the full set of variables as the memory vectors become non-sparse by the updating rule in \eqref{eq:alg2}. We resolve this issue by following the Just-in-Time approach in \cite{schmidt2017minimizing} and modifying \eqref{eq:alg2} to
% \begin{equation}\label{eq:alg2prime}
% \ba_t=\rho\frac{\bx_t-\bx_{t+1}}{\mu}-\alpha\left(\suml_n\bg_n+\suml_m\bh_m\right)_{I_t}
% \end{equation}
% where $I_t$ denotes the set of variables involved in the $t^\tth$ iteration and we define $(\by)_I$ for a vector $\by=(y_1,y_2,\ldots,y_d)$ as a vector $\by^\prime=(y_1^\prime,y_2^\prime,\ldots,y_d^\prime)$ such that
% \[
% y_i^\prime=\left\{\begin{array}{cc}
%     \frac{Ky_i}{K_i} & i\in I \\
%      0 & i\notin I
% \end{array}\right.
% \]
% where $K=M+N$ and $K_i$ is the number of objective terms $\phi_n$ and constraint sets $S_m$ including the $i^\tth$ variable $x_i$.


% \section{Just-in-Time (JiT) Update}
% Here we explain more details about the JiT procedure, explained in section 3.2. In our problem, each term $\phi_n(x)$ and constraint $S_m$ only involves a small subset $x_{I_n}:= (x_i, i \in I_n)$ of the variables, where $I_n \subseteq [d]$. Hence, the projection and proximal operators alter only a small subset of variables, dramatically reducing the amount of computation. We exploit this to give an algorithm that has much cheaper per-iteration cost. Note that the vanilla algorithm explained in \eqref{eq:alg1} and \eqref{eq:alg2} still operates on the full set of variables as the memory vectors become non-sparse by the updating rule in \eqref{eq:alg2}. We resolve this issue by following the Just-it-Time approach in [22] and modifying \eqref{eq:alg2} to
% \begin{equation}\label{eq:alg2prime}
% \ba_t=\rho\frac{\bx_t-\bx_{t+1}}{\mu}-\alpha\left(\suml_n\bg_n+\suml_m\bh_m\right)_{I_t}
% \end{equation}
% where $I_t$ denotes the set of variables involved in the $t^\tth$ iteration and we define $(\by)_I$ for a vector $\by=(y_1,y_2,\ldots,y_d)$ as a vector $\by^\prime=(y_1^\prime,y_2^\prime,\ldots,y_d^\prime)$ such that
% \[
% y_i^\prime=\left\{\begin{array}{cc}
%     \frac{Ky_i}{K_i} & i\in I \\
%      0 & i\notin I
% \end{array}\right.
% \]
% where $K=M+N$ and $K_i$ is the number of objective terms $\phi_n$ and constraint sets $S_m$ including the $i^\tth$ variable $x_i$.

% %In the projection step, we can use the sparse projection from \cite{Duch08}.

% % \section*{B -- Additional Experiments}

% % In this section, we report our additional numerical studies to investigate the different aspects of the proposed model. 

% % \subsection*{B -- 1 Early stopping of the optimization}

% % We study the early stopping of our  optimization procedure. We use  the data in Fig. \ref{fig:simple_synthetic_data_diverse} and investigate the results with different number of epochs. Here, we employ the OT-SON with proper parameterization, i.e., the results shown in the forth column and the second row for OT-SON in Fig.  \ref{fig:simple_synthetic_data_diverse}. In the experiments in Fig. \ref{fig:simple_synthetic_data_diverse} we performed the optimization with $20$ epochs. Here, we study early stopping, i.e., we study the quality of results if we stop after a smaller number of epochs. According to the results in Fig. \ref{fig:simple_synthetic_data_early_stopping}, we observe that even after a small number of epochs, we obtain reliable and stable results that represent well the ultimate solution. Such a property is very important in practice, as it can significantly reduce the heavy computations. Fig. \ref{fig:simple_synthetic_data_early_stopping_transport_map} illustrates the transport maps for different number of epochs. The different transport maps at different number of epochs are consistent with the transport cost shown in the last row of Fig. \ref{fig:simple_synthetic_data_early_stopping_transport_map}. 

% % \begin{figure*}[!ht]
% % \centering
% % \includegraphics[width=0.9\textwidth]{./3source2target/earlyStoppingDiagram10_5_withkernel_epochs7,10,12,15,17,20_witheponum}
% % \caption{Early stopping of the optimization after a finite number of epochs. The results are very consistent and stable even of we stop the algorithm very early.}
% % \label{fig:simple_synthetic_data_early_stopping}
% % \end{figure*}

% % \begin{figure*}[!ht]
% % \centering
% % \includegraphics[width=1\textwidth]{./3source2target/earlyStopping10_5_withkernel_epochs7,10,12,15,17,20_witheponum}
% % \caption{Consistency of the transport maps with the transport costs (shown at the last row) when using different finite number of epochs. Thus, early stopping can be useful for efficiency purposes. }
% % \label{fig:simple_synthetic_data_early_stopping_transport_map}
% % \end{figure*}



% % \subsection*{B -- 2 Diverse classes in the source}

% % We next study the case where two of the three source classes have the same label, as shown in Fig. \ref{fig:simple_synthetic_data_diverse_class}. In the source data (shown by yellow), the left and the middle data clouds have the same class labels. This example shows why the transport based on only the pairwise distances between the source and target data is insufficient. In Fig. \ref{fig:simple_synthetic_data_diverse_class}, the  left plot corresponds to $\lambda_1 = \lambda_2 =0$, the middle plot corresponds to $\lambda_1 = 10, \lambda_2 = 0.01$, and the right plot corresponds to $\lambda_1 = 100, \lambda_2 = 0.01$. We observe that the left plot (with $\lambda_1 = \lambda_2 =0$) fails to perform a proper transport of the source data. On the other hand, with incorporating our proposed regularization, the two different classes (even-though one of them is diverse) are properly transported to the target domain. We observe this kind of transfer in both of the middle ($\lambda_1 = 10, \lambda_2 = 0.01$) and right ($\lambda_1 = 100, \lambda_2 = 0.01$) plots. 

% % \begin{figure*}[!ht]
% % \centering
% % \includegraphics[width=0.333\textwidth]{./3source2target/TwoClassSameLabel0,0}
% % \hspace{-5mm}
% % \includegraphics[width=0.333\textwidth]{./3source2target/TwoClassSameLabel10,0_01noSim}
% % \hspace{-5mm}
% % \includegraphics[width=0.333\textwidth]{./3source2target/TwoClassSameLabel100,0_01withSim}
% % \caption{The impact of SON regularization when the class members are diverse. The plot in the left (where $\lambda_1 = \lambda_2 =0$) performs transportation solely based on pairwise distances, thus fails to transfer the classes properly. Our SON regularization (either $\lambda_1 = 10, \lambda_2 = 0.01$ or $\lambda_1 = 100, \lambda_2 = 0.01$) improves the transportation by enforcing block-specific transfers.}
% % \label{fig:simple_synthetic_data_diverse_class}
% % \end{figure*}

% % \subsection*{B -- 3 Fewer classes in the source}
% % In the experiments of Fig. \ref{fig:simple_synthetic_data_diverse}, we studied the case where the number of source classes is larger the number of target classes. Here, we consider an opposite setting: we assume two classes in the source and three classes in the target, as illustrated  in Fig. \ref{fig:simple_synthetic_data_diverse_2_3}. The source, target and transported data points are respectively shown by  yellow, blue, and red.  We use the same setting and parameters as in Fig. \ref{fig:simple_synthetic_data_diverse}, i.e., the first row corresponds to low regularization and the second row to high regularization (low regularization: $\lambda_1 = 0.01, \lambda_2=0.0$, high regularization: $\lambda_1 = 10, \lambda_2 = 5$). We observe that similar to the results in Fig. \ref{fig:simple_synthetic_data_diverse}, only OT-SON with high regularization prevents splitting the source data among all the three target classes. The last row in Fig. \ref{fig:simple_synthetic_data_diverse_2_3} indicates the consistency between the mapping costs and transport map for this setting (for OT-SON with high regularization).  

% % \begin{figure*}[t!]
% % \centering
% % \includegraphics[width=1\textwidth]{./3source2target/simple_emd_2_3}
% % %\includegraphics[width=0.24\textwidth]{./3source2target/simple_l1l2_mid}
% % %\includegraphics[width=0.24\textwidth]{./3source2target/simple_lpl1_mid}
% % %\includegraphics[width=0.24\textwidth]{./3source2target/simple_sinkhorn_mid}
% % %\includegraphics[width=0.24\textwidth]{./3source2target/simple_son_mid}
% % %\\
% % %\includegraphics[width=0.24\textwidth]{./3source2target/simple_l1l2_high}
% % %\includegraphics[width=0.24\textwidth]{./3source2target/simple_lpl1_high}
% % %\includegraphics[width=0.24\textwidth]{./3source2target/simple_sinkhorn_high}
% % %\includegraphics[width=0.24\textwidth]{./3source2target/10_5_withKernel}
% % \caption{Performance of different methods when the source has two classes and the target consists of three classes. The columns in order represent OT-l1l2, OT-lpl1, OT-Sinkhorn and OT-SON. Among different methods, only OT-SON with high regularization prevents splitting the source data among all the three target classes. The last row shows the consistency between the mapping costs and the transport map for OT-SON with high regularization.
% % %for OT-SON with this correct regularization.
% % }
% % \label{fig:simple_synthetic_data_diverse_2_3}
% % \end{figure*}




% %\subsection{Early stopping of the real-world experiments}
% %
% %\begin{figure*}[!ht]
% %\centering
% %\includegraphics[width=1\textwidth]{./3source2target/earlyStopping10_0_epochs1,5,10,15,20,mnistrm1,3,8}
% %\caption{Early Stopping on real2 with $\lambda_1 = 10, \lambda_2 = 0$. The bottom right picture is the transport cost}
% %\label{}
% %\end{figure*}

\section{Class Based Regularization}
\label{theory:class_based}
{\bf Asymptotic analysis for Gaussian Mixtures:} We start with a simplified probabilistic result for Gaussian mixtures in an asymptotic scenario, reflecting the main underlying intuitions of our analysis. We shortly present a more extensive study for finite and deterministic cases, which is also used for proving the first result:
\begin{figure}[t]
    \centering
    \includegraphics[width=.3\textwidth]{./Figure/clusters.png}
    \caption{An example of three pairs of Gaussian clusters in the source (blue) and target (red) domains. The maximum distance $d$ between associated (paired) centers, the minimum distance $D$ between unassociated centers and the maximum distance $E$ of centers between two domains are respectively shown by solid, dashed and dash-dotted lines.}
    \label{fig:ex}
\end{figure}
\begin{theorem}\label{thm:simp}
    Suppose in each of $K$ domains,  that an equal number $m$ of random real vectors are drawn from each of $K$ individual Gaussian distributions, leading to a total number of $n=mK$ samples. The Gaussian distributions in the source and target domains are respectively centered at $\btheta^s_\alpha,\btheta^t_\alpha$ for $\alpha=1,2,\ldots,K$, and all have uncorrelated entries with equal variance $\omega^2$. Squared $\ell_2$ distance is used, $d(\by_1,\by_2)=\|\by_1-\by_2\|_2^2$. With a probability higher than $1-\nicefrac{1}{n^{10}}$ the solution of \eqref{eq:framework} with a suitable choice of $\lambda$ classifies the samples of each Gaussian distribution, and associate the $\alpha^\tth$ distributions of the two domains for each $\alpha\in [K]$ if
    \begin{equation}\label{eq:cond_simp}
    \frac{D^2-d^2}{K\sqrt{K}}\geq C\sqrt{E^2+\omega^2}\log(nK),
    \end{equation}
    for some universal constant $C$, where $D=\min_{\alpha\neq\beta}\|\btheta^s_\alpha-\btheta^t_\beta\|$, $d=\max_{\alpha}\|\btheta^s_\alpha-\btheta^t_\alpha\|$ and $E=\max_{\alpha,\beta}\|\btheta^s_\alpha-\btheta^t_\beta\|$.
\end{theorem}
Fig. \ref{fig:ex} clarifies in a simple example the geometric meaning of the concepts used in the above result. As seen, the left hand side of the condition in \eqref{eq:cond_simp}, requires the associated clusters to be substantially closer to each other than the other clusters. Moreover, the right hand side of \eqref{eq:cond_simp} requires the distances to remain relatively bounded. An example of this situation is when $E,D,d\sim \sigma K\sqrt K\log(nK)$, i.e. all three grow proportionally with the number of samples, with a suitable proportion between them.

{\bf Deterministic Guarantee:} Now, we present an extended deterministic result that is used to prove theorem \ref{thm:simp}. We use a setting inspired by the stochastic block model. For simplicity, we describe here a model in which the data points in the source and target domains are each partitioned into $K$ parts with equal size $m$. We respectively denote the partitions in the source and target domains by $\{\mathscr{S}_\alpha\}$, $\{\mathscr{T}_\beta\}$. The total number of points in each domain is $n=mK$ (these assumptions are relaxed in Appendix B). Further, $\mathscr{S}_\alpha$ is paired with $\Delta_\alpha$ for every $\alpha\in [K]$. We investigate that the plan obtained by solving \eqref{eq:framework} consists of blocks, recovering both the sets of clusters $\{\mathscr{S}_\alpha\}$, $\{\mathscr{T}_\beta\}$ and their association. For this, we ensure that $X_{ij}$ remains zero for the $i^\tth$ data point in the source domain and $j^\tth$ data point in the target domain, belonging to unassociated clusters.  Accordingly, we require the \emph{ideal solution}  to be the one with $X_{i,j}=X_{\alpha,\beta}$ for $i\in \mathscr{S}_\alpha$ and $j\in \mathscr{T}_\beta$, where $X_{\alpha,\beta}$ are constants satisfying $X_{\alpha,\beta}=0$ for $\beta\neq\alpha$. 

For simplicity,  we take $S_{j,j^\prime}=1$ everywhere and study two cases where $R_{i,i^\prime}=1$ holds true either everywhere (no kernel) or for $i,i^\prime$ belonging to the same cluster and  $R_{i,i^\prime}=0$ otherwise  (perfect kernels in the source domain). The general case is presented in Appendix B. Introducing an indicator variable $R$, the first case is referred to by $R=0$ and the second one by $R=1$. Note also that we assume the optimization in \eqref{eq:framework} to be feasible for our ideal solution, which requires for every $i,i^\prime\in \mathscr{S}_\alpha$ and $j,j^\prime\in \mathscr{T}_\alpha$ that $\mu_i=\mu_{i^\prime}=\nu_j=\nu_{j^\prime}$. In Appendix B, we treat the general infeasible cases by considering a relaxation of \eqref{eq:framework}.

In the context of recovery  by the Kantorovich relaxation, a key concept is cyclical monotonicity \cite{villani2008optimal}, which we slightly modify and state below:
\begin{definition}	
We say that a set of coefficients $D_{\alpha,\alpha^\prime}$ for $\alpha,\alpha^\prime\in [K]$ satisfies the $\delta-$strong cyclical monotonicity condition if for each 
simple loop $\alpha_1\to \alpha_2\to \ldots \to \alpha_k\to \alpha_{k+1}=\alpha_1$ with length $k>1$ we have 
\begin{equation}\label{eq:strong_pos_loop_cond}
\suml_{l=1}^kD_{\alpha_l\alpha_{l+1}}> \suml_{l=1}^kD_{\alpha_l\alpha_{l}}+k\delta.
\end{equation}  
\end{definition}
Compared to the standard notion of cyclic monotonicity, we introduce a constant $\delta\geq 0$ in the right hand side of \eqref{eq:strong_pos_loop_cond}, which can be nonzero only when $(D_{\alpha,\beta})$ has a discrete or discontinuous nature. We apply this condition to the average distance of clusters given by 
$
D_{\alpha,\beta}= \frac{1}{m^2} \suml_{i\in \mathscr{S}_\alpha, j\in \mathscr{T}_\beta}D_{i,j}.
$
%Then, larger values of $\delta$ reflect better separation between clusters with respect to detecting the assignment $\pi$. Hence $\delta$ can be used as an empirical measure of separation between clusters (see the example below).   

% It is natural to expect an ideal solution only when the clusters are well-separated and $\delta$ is large, but the exact condition also requires a notion of metric in the two domains, which is not provided in the description of our problem. Our analysis introduces two different metrics: the first one is based on the geometric distance (cost) matrix $\bD$ and is used to provide the diameter of each cluster. The second one is based on the distributions $\bmu,\bnu$ and is used to assign a probabilistic distance or discrepancy between clusters. Our condition simply requires the maximal diameter of clusters to be relatively smaller than the product of the probabilistic and empirical ($\delta$) distance between the clusters in each domain.

%The geometric distance is simply obtained by respectively using the rows and columns of $\bD$ as embedding vectors for the data points in the source and target domain, and employing $\ell_2$ distance. This leads to $\nicefrac {\left\|\bd_i-\bd_{i^\prime}\right\|}{\sqrt{n}}$ and $\nicefrac {\left\|\bd^j-\bd^{j^\prime}\right\|}{\sqrt{n}}$ as the distance between source points $i,i^\prime$ and target points $j,j^\prime$, where again $\bd_i,\bd^j$ respectively refer to the rows and columns of $\bD$. The diameter of each cluster is the maximum distance between the points in that cluster and we denote by $\Delta$ the maximum diameter of the clusters in both domains.
We denote by $\Delta$ the maximum of the values $\nicefrac {\left\|\bd_i-\bd_{i^\prime}\right\|}{\sqrt{n}}$ and $\nicefrac {\left\|\bd^j-\bd^{j^\prime}\right\|}{\sqrt{n}}$ where source points $i,i^\prime$ and target points $j,j^\prime$ belong to the same cluster and we remind that $\bd_i,\bd^j$ respectively refer to the rows and columns of $\bD$.
%\begin{align}
%&\minl_{\bX\in \Pi(\bmu,\bnu)}\mathrm{Tr}(\bD^T\bX)+\nonumber \\
%&\qquad \lambda\left(\suml_{l,k} R_{l,k}\|\bx_l-\bx_k\|_2+\suml_{l,k} S_{l,k}\|\bx^l-\bx^k\|_2\right)+ \nonumber \\
%&\qquad \frac\theta 2\left(\|\bX\bone-\bmu\|_2^2+\|\bX^T\bone-\bnu\|_2^2\right),
%\end{align}
%where $\theta$ is a design parameter. Here, we focus on \eqref{eq:framework} under feasibility assumptions. 
We also  define
$
\omega_\alpha :=\suml_{i\in \mathscr{S}_\alpha}\mu_i=\suml_{j\in D_{\alpha}}\nu_j
$
and then take $T_{\alpha,\beta}=\suml_{\gamma\in [K]}
\left(\frac{R\omega_\alpha}{\sqrt{\omega_\alpha^2+\omega_\gamma^2}}+
\frac{\omega_\beta}{\sqrt{\omega_\beta^2+\omega_\gamma^2}}
\right)-\frac{1+R}{\sqrt 2}$
. Finally, we define
\[
\Lambda_{\alpha,\beta}= \left(
%\frac{1+R}{2}T_{\alpha,\beta}+
T_{\alpha,\beta}+
\frac{\omega_\alpha+R\omega_\beta}{\sqrt{\omega_\beta^2+\omega_\beta^2}} \right)^{-1},
\]
and take $\Lambda$ as its maximum over $\alpha\neq\beta$. Accordingly, we obtain the following result:
%This number reflects the amount of "unbalancedness" in the measure $\omega_{\alpha}$ (See the example below). Then, we have the following result:
\begin{theorem}
\label{thm:guarantee}
Suppose that
$(D_{\alpha,\beta})$ is $\delta-$strongly cyclical monotone. Take $\lambda$ such that $\Delta \leq \lambda\sqrt{\nicefrac{m}{K}}$. Then, the solution of \eqref{eq:framework} is given by $X_{ij}=X_{\alpha,\beta}$ for $i\in \mathscr{S}_\alpha$ and $j\in \mathscr{T}_\beta$ satisfying one of the following two conditions:
\begin{enumerate}
\item We have $X_{\alpha,\beta}=\nicefrac{\omega_\alpha}{m^2}\delta_{\beta,\alpha}$ if 
$
\Delta\sqrt{K}\leq\lambda\sqrt{m}
\leq \Lambda\delta
$
\item Otherwise, we have
$
\delta\suml_{\beta\neq \alpha}X_{\alpha,\beta}\leq
\lambda(1+R)\sqrt m\suml_{\alpha\neq\alpha^\prime}
\sqrt{\omega^2_\alpha+\omega^2_{\alpha^\prime}
}.
$
\end{enumerate}
Furthermore, the solution is unique in part 1 if all inequalities are strict.
\begin{proof}
Proof can be found in section \ref{proof:guarantee}.
\end{proof}
\end{theorem}
The first part of theorem \ref{thm:guarantee} establishes ideal recovery under the condition that the "effective cluster diameter" $\Delta$ is relatively smaller than $\Lambda\delta$. The second part gives an upper bound on the error $\suml_{\beta\neq \alpha}X_{\alpha,\beta}$. Note that $\Delta$ is always smaller with $R=1$ compared to $R=0$, making the conditions less restrictive. This reflects the intuitive fact that introducing kernels simplifies the estimation process.

{\bf Proof of Theorem \ref{thm:simp}:} Based on theorem \ref{thm:guarantee}, we present a sketch of the proof for theorem \ref{thm:simp}. Under the assumptions of theorem \ref{thm:simp}, we directly verify that $\delta=D^2-d^2$ is a valid choice. Moreover $\Lambda=\Lambda_{\alpha,\beta}=\nicefrac{\sqrt 2}{K(1+R)}$. Finally, we may conclude by Chernoff bound that with a probability exceeding $1-\nicefrac 1{n^{10}}$ (the power 10 is arbitrary) we have $\Delta=O(\sqrt{E^2+\omega^2}\log(nK))$. Replacing these expression in the first part of theorem \ref{thm:guarantee} gives us the result.
%{\bf Example:}  Suppose that each domain consists of two clusters of data points on $\bbR^b$ each generated by a Gaussian distribution with equal variance $\omega^2$. We denote the mean of the $\alpha^\tth$ cluster from $k^\tth$ domain for $\alpha=1,2$ and $k=1,2$ by $\bmu_\alpha^j$. We take $\pi(1)=1,\pi(2)=2$ and define the distance matrix as the square $\ell_2$ distance of the points in two different domains. We denote by $\rho$ the minimum of mean point distances in similar domains, i.e $\|\bmu^k_1-\bmu^k_2\|$, and take $d$ as their maximum between domains, i.e. $d_{\alpha,\beta}=\|\bmu_\alpha^1-\bmu_\beta^2\|$. By triangle inequality, $\rho\leq 2d$. We take no kernel, i.e. $R=1$.

%In this case, we observe that $\Lambda=\nicefrac{\sqrt{\omega_1^2+\omega_2^2}}{3(\omega_1+\omega_2)}$ and hence $1/3\sqrt{2}\leq\Lambda\leq 1/3$, where $\Lambda$ reaches its maximum value for highly unbalanced measures $\omega_2/\omega_1\to 0$ or $\infty$. This confirms that $\Lambda$ is a figure of variability among clusters. We observe that $\Delta=O(\sqrt{d^2+\omega^2}\log  n)$ with a probability of at east $1-\nicefrac{1}{n^{10}}$ \footnote{The power of $10$ is arbitrary.}. Theorem \ref{thm:guarantee} in this case implies that there exists a constant $C$ such that with the same probability our approach recovers the clusters and $\pi$ if
% \[
% \delta=\frac{d_{11}^2+d_{22}^2-d_{12}^2-d_{21}^2}2\geq C\sqrt{d^2+\omega^2}\log n
% \]
% We notice that $\delta$ is the difference between the average distance $d_{11}^2+d_{22}^2$ of corresponding clusters by $\pi$ and the average distance $d_{12}^2+d_{21}^2$ of unassociated ones. Hence, the above condition means that each cluster in the target domain is substantially closer, on average, to its corresponding cluster in the source domain. This condition also imposes the clusters to be geometrically well-separated in each domain. To see this from triangle inequality, we observe that $\delta\leq 2d\rho-\rho^2$ and hence, we also require that $2d\rho-\rho^2\geq C\sqrt{d^2+\omega^2}\log n$, implying $\rho\geq C/2\log n$, i.e. well-separated centers.



